Bitangents to symmetric quartics

Recall that a non-singular planar quartic is a canonically embedded non-hyperelliptic curve of genus three. We say such a curve is symmetric if it admits non-trivial automorphisms. The classification of (necessarily finite) groups appearing as automorphism groups of non-singular curves of genus three dates back to the last decade of the 19th century. As these groups act on the quartic via projective linear transformations, they induce symmetries on the 28 bitangents. Given such an automorphism group $G=\mathrm{Aut}(C)$, we prove the $G$-orbits of the bitangents are independent of the choice of $C$, and we compute them for all twelve types of smooth symmetric planar quartic curves. We further observe that techniques deriving from equivariant homotopy theory directly reveal patterns which are not obvious from a classical moduli perspective.

==> commands.tex <==
\RequirePackage{amsmath,amssymb,amsthm}
\RequirePackage{amsfonts}
\RequirePackage{color}
\RequirePackage{tikz}
\RequirePackage{tikz-cd}
\RequirePackage{hyperref}

% Formatting
\usepackage[margin=1in]{geometry}
\setlength{\parindent}{0pt}
\setlength{\parskip}{0.5em}



\usepackage{enumitem}[cleveref]
\usepackage{amsfonts}
\usepackage{float}


% For arrows
\RequirePackage{mathtools}

% For script letters
\RequirePackage{mathrsfs}

\usepackage{color}
\newcommand{\todo}{\color{red}{todo}\hspace{0.5em}\color{black}}


% Custom-common.sty
% Built by tbrazel/latex-templates/

\RequirePackage{amsmath,amssymb,amsthm}
\RequirePackage{amsfonts}
\RequirePackage{color}
\RequirePackage{tikz}
\RequirePackage{tikz-cd}

% For arrows
\RequirePackage{mathtools}

% For script letters
\RequirePackage{mathrsfs}
%%%%%%%%%%%%
% arrows
%%%%%%%%%%%
% Arrows
\RequirePackage{mathtools}

% Pushout, pullback
\providecommand{\po}{\arrow[ul,phantom,"\ulcorner" very near start]}
\providecommand{\pb}{\arrow[dr,phantom,"\lrcorner" very near start]}
\providecommand{\xto}[1]{\xrightarrow{#1}}
\providecommand{\from}{\leftarrow}
\providecommand{\xfrom}[1]{\overset{#1}{\leftarrow}}

\providecommand{\mapsfrom}{\mathrel{\reflectbox{\ensuremath{\mapsto}}}}
\providecommand{\longmapsfrom}{\mathrel{\reflectbox{\ensuremath{\longmapsto}}}}

\providecommand{\hookto}{\xhookrightarrow{}}
\providecommand{\xhookto}[1]{\overset{#1}{\hookrightarrow}}

\providecommand{\hookfrom}{\xhookleftarrow{}}
\providecommand{\xhookfrom}[1]{\xhookleftarrow{#1}}

\providecommand{\tto}{\twoheadrightarrow}
\providecommand{\xtto}[1]{\overset{#1}{\twoheadrightarrow}}
\providecommand{\ffrom}{\twoheadleftarrow}
\providecommand{\xffrom}[1]{\overset{#1}{\ffrom}}

\providecommand{\ladjoint}[2]{ #1\rightleftarrows #2 }
\makeatletter
\providecommand{\superimpose}[2]{%
  {\ooalign{$#1\@firstoftwo#2$\cr\hfil$#1\@secondoftwo#2$\hfil\cr}}}
\makeatother
\providecommand{\smallslash}{\mbox{\tiny/}}

\providecommand{\clhookto}{\mathrel{\raisebox{0.1em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.1em}\smallslash}{\hookrightarrow}}}$}}}
\providecommand{\xclhook}[1]{\overset{#1}{\clhook}}

\providecommand{\clhookfrom}{\mathrel{\raisebox{0.1em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.1em}\smallslash}{\hookleftarrow}}}$}}}

\providecommand{\ohookto}{\mathrel{\raisebox{0.03em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.03em}\mbox{\small$\circ$}}{\hookrightarrow}}}$}}}

\providecommand{\ohookfrom}{\mathrel{\raisebox{0.03em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.03em}\mbox{\small$\circ$}}{\hookleftarrow}}}$}}}

% Cofibrations
\providecommand{\cofto}{\rightarrowtail}
\providecommand{\coffrom}{\leftarrowtail}
\providecommand{\xcofto}[1]{\overset{#1}{\cofto}}
\providecommand{\xcoffrom}[1]{\overset{#1}{\coffrom}}

% Dashed arrows
\providecommand{\dashto}{\dashrightarrow}
\providecommand{\dashfrom}{\dashleftarrow}


%%%%%%%%%%%%%
% Text commands
\providecommand{\ab}{\text{ab}}
\providecommand{\alg}{\text{alg}}
\providecommand{\ann}{\text{ann}}
\providecommand{\Aut}{\text{Aut}}
\providecommand{\BG}{\text{BG}}
\providecommand{\BGL}{\text{BGL}}
\providecommand{\Bl}{\text{Bl}}
\providecommand{\BO}{\text{BO}}
\providecommand{\BP}{\text{BP}}
\providecommand{\BSL}{\text{BSL}}
\providecommand{\BSO}{\text{BSO}}
\providecommand{\BSp}{\text{BSp}}
\providecommand{\BSU}{\text{BSU}}
\providecommand{\BU}{\text{BU}}
\providecommand{\can}{\text{can}}
\providecommand{\cd}{\text{cd}}
\providecommand{\cdh}{\text{cdh}}
\providecommand{\char}{\text{char}}
\providecommand{\cl}{\text{cl}}
\providecommand{\codim}{\text{codim}}
\providecommand{\codom}{\text{codom}}
\providecommand{\coeq}{\text{coeq}}
\providecommand{\coev}{\text{coev}}
\providecommand{\cof}{\text{cof}}
\providecommand{\cofib}{\text{cofib}}
\providecommand{\coker}{\text{coker}}
\providecommand{\colim}{\text{colim}}
\providecommand{\cone}{\text{cone}}
\providecommand{\conj}{\text{conj}}
\providecommand{\const}{\text{const}}
\providecommand{\cyc}{\text{cyc}}
\providecommand{\dg}{\text{dg}}
\providecommand{\Disc}{\text{Disc}}
\providecommand{\disc}{\text{disc}}
\providecommand{\dual}{\text{dual}}
\providecommand{\eff}{\text{eff}}
\providecommand{\EKL}{\text{EKL}}
\providecommand{\End}{\text{End}}
\providecommand{\eq}{\text{eq}}
\providecommand{\et}{\text{et}}
\providecommand{\EU}{\text{EU}}
\providecommand{\ev}{\text{ev}}
\providecommand{\Ex}{\text{Ex}}
\providecommand{\ex}{\text{ex}}
\providecommand{\Exc}{\text{Exc}}
\providecommand{\Ext}{\text{Ext}}
\providecommand{\fib}{\text{fib}}
\providecommand{\Fix}{\text{Fix}}
\providecommand{\Frac}{\text{Frac}}
\providecommand{\Frob}{\text{Frob}}
\providecommand{\Fun}{\text{Fun}}
\providecommand{\Gal}{\text{Gal}}
\providecommand{\gen}{\text{gen}}
\providecommand{\GL}{\text{GL}}
\providecommand{\gp}{\text{gp}}
\providecommand{\Gr}{\text{Gr}}
\providecommand{\gr}{\text{gr}}
\providecommand{\GW}{\text{GW}}
\providecommand{\Her}{\text{Her}}
\providecommand{\Ho}{\text{Ho}}
\providecommand{\hocofib}{\text{hocofib}}
\providecommand{\hocolim}{\text{hocolim}}
\providecommand{\hofib}{\text{hofib}}
\providecommand{\holim}{\text{holim}}
\providecommand{\Hom}{\text{Hom}}
\providecommand{\id}{\text{id}}
\providecommand{\Idem}{\text{Idem}}
\providecommand{\im}{\text{im}}
\providecommand{\incl}{\text{incl}}
\providecommand{\Ind}{\text{Ind}}
\providecommand{\inj}{\text{inj}}
\providecommand{\Inn}{\text{Inn}}
\providecommand{\inv}{\text{inv}}
\providecommand{\iso}{\text{iso}}
\providecommand{\Jac}{\text{Jac}}
\providecommand{\KGL}{\text{KGL}}
\providecommand{\kgl}{\text{kgl}}
\providecommand{\KH}{\text{KH}}
\providecommand{\KO}{\text{KO}}
\providecommand{\ko}{\text{ko}}
\providecommand{\KQ}{\text{KQ}}
\providecommand{\kq}{\text{kq}}
\providecommand{\KR}{\text{KR}}
\providecommand{\KSp}{\text{KSp}}
\providecommand{\KU}{\text{KU}}
\providecommand{\ku}{\text{ku}}
\providecommand{\Lan}{\text{Lan}}
\providecommand{\Map}{\text{Map}}
\providecommand{\map}{\text{map}}
\providecommand{\MGL}{\text{MGL}}
\providecommand{\MO}{\text{MO}}
\providecommand{\Mor}{\text{Mor}}
\providecommand{\mor}{\text{mor}}
\providecommand{\MSL}{\text{MSL}}
\providecommand{\MSO}{\text{MSO}}
\providecommand{\MSp}{\text{MSp}}
\providecommand{\MSU}{\text{MSU}}
\providecommand{\MU}{\text{MU}}
\providecommand{\mult}{\text{mult}}
\providecommand{\ob}{\text{ob}}
\providecommand{\obj}{\text{obj}}
\providecommand{\op}{\text{op}}
\providecommand{\Orb}{\text{Orb}}
\providecommand{\ord}{\text{ord}}
\providecommand{\Out}{\text{Out}}
\providecommand{\perf}{\text{perf}}
\providecommand{\Perm}{\text{Perm}}
\providecommand{\PGL}{\text{PGL}}
\providecommand{\Pr}{\text{Pr}}
\providecommand{\pr}{\text{pr}}
\providecommand{\pre}{\text{pre}}
\providecommand{\Proj}{\text{Proj}}
\providecommand{\proj}{\text{proj}}
\providecommand{\PSL}{\text{PSL}}
\providecommand{\quot}{\text{quot}}
\providecommand{\Ran}{\text{Ran}}
\providecommand{\rank}{\text{rank}}
\providecommand{\Res}{\text{Res}}
\providecommand{\RO}{\text{RO}}
\providecommand{\sep}{\text{sep}}
\providecommand{\sgn}{\text{sgn}}
\providecommand{\SH}{\text{SH}}
\providecommand{\sig}{\text{sig}}
\providecommand{\Sing}{\text{Sing}}
\providecommand{\SL}{\text{SL}}
\providecommand{\SO}{\text{SO}}
\providecommand{\soc}{\text{soc}}
\providecommand{\Sp}{\text{Sp}}
\providecommand{\Span}{\text{Span}}
\providecommand{\Spin}{\text{Spin}}
\providecommand{\spn}{\text{spn}}
\providecommand{\Sq}{\text{Sq}}
\providecommand{\st}{\text{st}}
\providecommand{\Stab}{\text{Stab}}
\providecommand{\SU}{\text{SU}}
\providecommand{\supp}{\text{supp}}
\providecommand{\Syl}{\text{Syl}}
\providecommand{\syl}{\text{syl}}
\providecommand{\Sym}{\text{Sym}}
\providecommand{\syn}{\text{syn}}
\providecommand{\SYT}{\text{SYT}}
\providecommand{\TC}{\text{TC}}
\providecommand{\td}{\text{td}}
\providecommand{\Th}{\text{Th}}
\providecommand{\THH}{\text{THH}}
\providecommand{\Tor}{\text{Tor}}
\providecommand{\TP}{\text{TP}}
\providecommand{\TR}{\text{TR}}
\providecommand{\Tr}{\text{Tr}}
\providecommand{\tr}{\text{tr}}
\providecommand{\univ}{\text{univ}}
\providecommand{\veff}{\text{veff}}
\providecommand{\vol}{\text{vol}}
\providecommand{\Wel}{\text{Wel}}
\providecommand{\Wr}{\text{Wr}}

% Special text commands
\providecommand{\et}{\text{\'{e}t}}
\renewcommand{\Im}{\text{Im}}
\renewcommand{\Re}{\text{Re}}
\providecommand{\Spec}{\text{Spec}\hspace{0.1em}}
\providecommand{\spn}{\text{span}}

% Blackboard letters
\providecommand{\A}{\mathbb{A}}
\providecommand{\C}{\mathbb{C}}
\providecommand{\F}{\mathbb{F}}
\providecommand{\G}{\mathbb{G}}
\providecommand{\H}{\mathbb{H}}
\providecommand{\N}{\mathbb{N}}
\providecommand{\P}{\mathbb{P}}
\providecommand{\Q}{\mathbb{Q}}
\providecommand{\R}{\mathbb{R}}
\providecommand{\Z}{\mathbb{Z}}

%%%%%%%%%%%%%Colors
\usepackage{xcolor}
\definecolor{darkgreen}{rgb}{0,0.30,0}
\definecolor{darkred}{rgb}{0.75,0,0}
\definecolor{darkblue}{rgb}{0,0,0.6}
%%%%%%%%%%%%
% shorthand
% Common shorthands
\let\til\widetilde
\let\nsubgp\trianglelefteq
\let\emptyset\varnothing
% AT commands
\providecommand{\BG}{\text{BG}}
\providecommand{\BO}{\text{BO}}
\providecommand{\BP}{\text{BP}}
\providecommand{\BU}{\text{BU}}
\providecommand{\BSL}{\text{BSL}}
\providecommand{\BSO}{\text{BSO}}
\providecommand{\BSU}{\text{BSU}}
\providecommand{\BGL}{\text{BGL}}
\providecommand{\coeq}{\text{coeq}}
\providecommand{\cof}{\text{cof}}
\providecommand{\cone}{\text{cone}}
\providecommand{\eq}{\text{eq}}
\providecommand{\EU}{\text{EU}}
\providecommand{\Ex}{\text{Ex}}
\providecommand{\Ext}{\text{Ext}}
\providecommand{\Gr}{\text{Gr}}
\providecommand{\Ho}{\text{Ho}}
\providecommand{\hocofib}{\text{hocofib}}
\providecommand{\hocolim}{\text{hocolim}}
\providecommand{\holim}{\text{holim}}
\providecommand{\KGL}{\text{KGL}}
\providecommand{\KH}{\text{KH}}
\providecommand{\ko}{\text{ko}}
\providecommand{\KO}{\text{KO}}
\providecommand{\kq}{\text{kq}}
\providecommand{\KQ}{\text{KQ}}
\providecommand{\KR}{\text{KR}}
\providecommand{\KSp}{\text{KSp}}
\providecommand{\ku}{\text{ku}}
\providecommand{\KU}{\text{KU}}
\providecommand{\Lan}{\text{Lan}}
\providecommand{\MGL}{\text{MGL}}
\providecommand{\MO}{\text{MO}}
\providecommand{\MSL}{\text{MSL}}
\providecommand{\MSO}{\text{MSO}}
\providecommand{\MSp}{\text{MSp}}
\providecommand{\MSU}{\text{MSU}}
\providecommand{\MU}{\text{MU}}
\providecommand{\Out}{\text{Out}}
\providecommand{\pre}{\text{pre}}
\providecommand{\Ran}{\text{Ran}}
\providecommand{\RO}{\text{RO}}
\providecommand{\Sing}{\text{Sing}}
\providecommand{\SO}{\text{SO}}
\providecommand{\Spin}{\text{Spin}}
\providecommand{\Sq}{\text{Sq}}
\providecommand{\SU}{\text{SU}}
\providecommand{\Sym}{\text{Sym}}
\providecommand{\TC}{\text{TC}}
\providecommand{\Th}{\text{Th}}
\providecommand{\THH}{\text{THH}}
\providecommand{\TP}{\text{TP}}
\providecommand{\TR}{\text{TR}}
\providecommand{\SH}{\mathcal{SH}}
\providecommand{\Sp}{\textit{Sp}}
\providecommand{\veff}{\text{veff}}


% Chromatic
\providecommand{\Prin}{\text{Prin}}
\providecommand{\FGL}{\text{FGL}}
\providecommand{\SI}{\text{SI}}
\providecommand{\FG}{\text{FG}}
\providecommand{\fg}{\text{fg}}




% Spaces
\providecommand{\CP}{{\mathbb{C}\text{P}}}
\providecommand{\HP}{{\mathbb{H}\text{P}}}
\providecommand{\RP}{{\mathbb{R}\text{P}}}

% EM Spectra
\providecommand{\HF}{{\text{H}\mathbb{F}}}
\providecommand{\HQ}{{\text{H}\mathbb{Q}}}
\providecommand{\HZ}{{\text{H}\mathbb{Z}}}

% Other
\providecommand{\Cech}{\check{C}}
\let\adj\dashv
\let\smashprod\wedge


% custom-cats.sty

% Categories
\providecommand{\Ab}{\text{Ab}}
\providecommand{\Alg}{\text{Alg}}
\providecommand{\Ani}{\text{Ani}}
\providecommand{\Bimod}{\text{Bimod}}
\providecommand{\CAlg}{\text{CAlg}}
\providecommand{\Cat}{\text{Cat}}
\providecommand{\CDGA}{\text{CDGA}}
\providecommand{\CG}{\text{CG}}
\providecommand{\CGWH}{\text{CGWH}}
\providecommand{\Ch}{\text{Ch}}
\providecommand{\CMon}{\text{CMon}}
\providecommand{\coAlg}{\text{coAlg}}
\providecommand{\Coh}{\text{Coh}}
\providecommand{\CommRing}{\text{CommRing}}
\providecommand{\ConjSub}{\text{ConjSub}}
\providecommand{\coMod}{\text{coMod}}
\providecommand{\Cor}{\text{Cor}}
\providecommand{\Corr}{\text{Corr}}
\providecommand{\CoSh}{\text{CoSh}}
\providecommand{\CRing}{\text{CRing}}
\providecommand{\CW}{\text{CW}}
\providecommand{\Field}{\text{Field}}
\providecommand{\Fin}{\text{Fin}}
\providecommand{\FinSet}{\text{FinSet}}
\providecommand{\Gpd}{\text{Gpd}}
\providecommand{\Grp}{\text{Grp}}
\providecommand{\Grpd}{\text{Grpd}}
\providecommand{\Grph}{\text{Grph}}
\providecommand{\Kan}{\text{Kan}}
\providecommand{\Kar}{\text{Kar}}
\providecommand{\LMod}{\text{LMod}}
\providecommand{\Mfld}{\text{Mfld}}
\providecommand{\Mod}{\text{Mod}}
\providecommand{\NAlg}{\text{NAlg}}
\providecommand{\Ouv}{\text{Ouv}}
\providecommand{\Perf}{\text{Perf}}
\providecommand{\Poset}{\text{Poset}}
\providecommand{\Pr}{\text{Pr}}
\providecommand{\Pre}{\text{Pre}}
\providecommand{\PSh}{\text{PSh}}
\providecommand{\PShv}{\text{PShv}}
\providecommand{\qCat}{\text{qCat}}
\providecommand{\QCoh}{\text{QCoh}}
\providecommand{\Rep}{\text{Rep}}
\providecommand{\Ring}{\text{Ring}}
\providecommand{\RMod}{\text{RMod}}
\providecommand{\sAb}{\text{sAb}}
\providecommand{\Set}{\text{Set}}
\providecommand{\SH}{\text{SH}}
\providecommand{\Sh}{\text{Sh}}
\providecommand{\Shv}{\text{Shv}}
\providecommand{\Sp}{\text{Sp}}
\providecommand{\Spectra}{\text{Spectra}}
\providecommand{\sPre}{\text{sPre}}
\providecommand{\sSet}{\text{sSet}}
\providecommand{\sShv}{\text{sShv}}
\providecommand{\Stack}{\text{Stack}}
\providecommand{\Sub}{\text{Sub}}
\providecommand{\Top}{\text{Top}}
\providecommand{\Vect}{\text{Vect}}

%%%%%%%%%%%%
% category_theory
% For blackboard bold number and delta categories
\RequirePackage{bbm}
\providecommand{\onecat}{\mathbbm{1}}
\providecommand{\twocat}{\mathbbm{2}}

% Blackboard delta
\RequirePackage{pict2e,picture}

\makeatletter
\DeclareRobustCommand{\DDelta}{{\mathpalette\bb@Delta\relax}}
\newcommand{\bb@Delta}[2]{%
  \begingroup
  \sbox\z@{$\m@th#1\Delta$}%
  \dimendef\Dht=6 \dimendef\Dwd=8
  \setlength{\Dwd}{\wd\z@}%
  \setlength{\Dht}{\ht\z@}%
  \begin{picture}(\Dwd,\Dht)
  \put(0,0){$\m@th#1\Delta$}
  \put(.42\Dwd,.7\Dht){\line(10,-26){.25\Dht}}
  \end{picture}%
  \endgroup
}


% Heart (for e.g. t-structures)
\usepackage{graphicx}
\newcommand{\heart}{\ensuremath\heartsuit}

\RequirePackage{amsmath,amssymb}

% Mis
\providecommand{\A}{\mathbb{A}}
\providecommand{\Gm}{\mathbb{G}_m}


% Text commands
\providecommand{\CH}{\text{CH}}
\providecommand{\CHW}{\widetilde{\text{CH}}}
\providecommand{\DM}{\text{DM}}
\providecommand{\et}{\text{\'{e}t}}
\providecommand{\mot}{\text{mot}}
\providecommand{\MW}{\text{MW}}
\providecommand{\Nis}{\text{Nis}}
\providecommand{\RS}{\text{RS}}
\providecommand{\Sing}{\text{Sing}}
\providecommand{\Zar}{\text{Zar}}

% Categories
\providecommand{\SH}{\text{SH}}
\providecommand{\Sm}{\text{Sm}}
\providecommand{\Spc}{\text{Spc}}
\providecommand{\Spt}{\text{Spt}}

% Spectra
\providecommand{\HZ}{\text{H}\mathbb{Z}}
\providecommand{\KGL}{\text{KGL}}
\providecommand{\KH}{\text{KH}}
\providecommand{\KO}{\text{KO}}
\providecommand{\KQ}{\text{KQ}}
\providecommand{\MGL}{\text{MGL}}
\providecommand{\MSL}{\text{MSL}}
\providecommand{\MSLc}{\text{MSL}^c}

\RequirePackage{amsmath,amsthm,thmtools}
\RequirePackage{cleveref}
\let\fullref\autoref
%

\def\makeautorefname#1#2{\expandafter\def\csname#1autorefname\endcsname{#2}}

%  
\makeautorefname{assump}{assumption}%
\makeautorefname{cla}{claim}%
\makeautorefname{conj}{conjecture}%
\makeautorefname{cor}{corollary}%
\makeautorefname{cex}{counterexample}%
\makeautorefname{cexs}{counterexamples}%
\makeautorefname{code}{codeblock}%
\makeautorefname{data}{data}%
\makeautorefname{dig}{digression}%
\makeautorefname{disc}{discussion}%
\makeautorefname{def}{definition}%
\makeautorefname{ex}{example}%
\makeautorefname{exs}{examples}%
\makeautorefname{fac}{fact}%
\makeautorefname{intu}{intuition}%
\makeautorefname{lem}{lemma}%
\makeautorefname{meta}{metathm}%
\makeautorefname{nota}{notation}%
\makeautorefname{note}{note}%
\makeautorefname{prop}{proposition}%
\makeautorefname{ques}{question}%
\makeautorefname{rmk}{remark}%
\makeautorefname{term}{terminology}%
\makeautorefname{thm}{theorem}%
\makeautorefname{upsh}{upshot}%
\makeautorefname{warn}{warn}%

\makeautorefname{eqn}{Equation}%
\makeautorefname{fig}{Figure}%
\makeautorefname{sec}{Section}%
\makeautorefname{subsec}{Subsection}%

% Theorem environments
\theoremstyle{definition}
\newtheorem{theorem}{Theorem}[section]

\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{codeblock}[theorem]{Codeblock}
\newtheorem{computation}[theorem]{Computation}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{counterexample}[theorem]{Counterexample}
\newtheorem{data}[theorem]{Data}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{digression}[theorem]{Digression}
\newtheorem{example}[theorem]{Example}
\newtheorem{examples}[theorem]{Examples}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{idea}[theorem]{Idea}
\newtheorem{intuition}[theorem]{Intuition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{metathm}[theorem]{Meta-theorem}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{note}[theorem]{Note}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{question}[theorem]{Question}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{slogan}[theorem]{Slogan}
\newtheorem{strategy}[theorem]{Strategy}
\newtheorem{terminology}[theorem]{Terminology}
\newtheorem{upshot}[theorem]{Upshot}
\newtheorem{warn}[theorem]{Warning}

%\newtheorem{warning}[theorem]{Warning}

%%%% hack to get fullref working correctly
\makeatletter
\let\c@corollary=\c@theorem
\let\c@proposition=\c@theorem
\let\c@lemma=\c@theorem
\let\c@assumption=\c@theorem
\let\c@conjecture=\c@theorem
\let\c@definition=\c@theorem
\let\c@example=\c@theorem
\let\c@remark=\c@theorem
\let\c@notation=\c@theorem
\let\c@equation\c@theorem
\makeatother

\renewcommand*{\subsectionautorefname}{Subsection}
\renewcommand*{\sectionautorefname}{Section}


\RequirePackage{amsmath,amssymb}

% AG commands
\providecommand{\aff}{\text{aff}}
\providecommand{\Ann}{\text{Ann}}
\providecommand{\Alt}{\text{Alt}}
\providecommand{\Cl}{\text{Cl}}
\renewcommand{\div}{\text{div}}
\providecommand{\Div}{\text{Div}}
\providecommand{\Frob}{\text{Frob}}
\providecommand{\Gr}{\text{Gr}}
\providecommand{\Krulldim}{\text{Krulldim}}
\providecommand{\Max}{\text{Max}}
\providecommand{\nil}{\text{nil}}
\providecommand{\nr}{\text{nr}}
\providecommand{\Pic}{\text{Pic}}
\providecommand{\Proj}{\text{Proj}\hspace{0.1em}}
\providecommand{\PSh}{\text{PSh}}
\providecommand{\red}{\text{red}}
\providecommand{\sm}{\text{sm}}
\providecommand{\Sh}{\text{Sh}}
\providecommand{\Spec}{\text{Spec}\hspace{0.1em}}
\providecommand{\Specmax}{\text{Specmax}\hspace{0.1em}}
\providecommand{\Sym}{\text{Sym}}
\providecommand{\trdeg}{\textit{tr}.\textit{deg}\hspace{0.1em}}
\providecommand{\Val}{\text{Val}}
\providecommand{\Var}{\text{Var}}
\providecommand{\Zar}{\text{Zar}}

% AG Categories
\providecommand{\Aff}{\text{Aff}}
\providecommand{\AffVar}{\text{AffVar}}
\providecommand{\Coh}{\text{QCoh}}
\providecommand{\QCoh}{\text{Coh}}
\providecommand{\Sch}{\text{Sch}}
\providecommand{\preVar}[1]{\text{preVar}\text{-}#1}
% AG Symbols
\providecommand{\A}{\mathbb{A}}
\providecommand{\Gm}{\mathbb{G}_{\text{m}}}
\providecommand{\m}{\mathfrak{m}}
\renewcommand{\O}{\mathscr{O}}
\providecommand{\p}{\mathfrak{p}}
\renewcommand{\P}{\mathbb{P}}
\providecommand{\q}{\mathfrak{q}}

% AG Arrows
\providecommand{\dashto}{\dashrightarrow}
\providecommand{\dashfrom}{\mathrel{\reflectbox{\ensuremath{\dashrightarrow}}}}

\let\und\underline



